Stability of parabolic Harnack inequalities on metric measure spaces

Let $(X,d,\mu)$ be a metric measure space with a local regular Dirichlet form. We give necessary and sufficient conditions for a parabolic Harnack inequality with global space-time scaling exponent $\beta\ge 2$ to hold. We show that this parabolic Harnack inequality is stable under rough isometries. As a consequence, once such a Harnack inequality is established on a metric measure space, then it holds for any uniformly elliptic operator in divergence form on a manifold naturally defined from the graph approximation of the space.

==> bbk-correct2020-fin.tex <==
%MB 16.1.2020

\magnification 1200
\hsize=17 truecm  
\vsize=8.5  truein
\baselineskip=15 truept

\def\bigb{\bigbreak\noindent}         
\def\med{\medbreak\noindent}
\def\small{\smallskip\noindent}
\def\nl{\hfil\break}
\def\no{\noindent}

\def\today{\noindent\number\day
\space\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\year}

\def\cl {\centerline}
\def\i {\item}
\def\ii {\itemitem}

\input amssym.def
\input amssym.tex
\input epsf

\def\bP {{\Bbb P}} \def\bE {{\Bbb E}} \def\Q {{\Bbb Q}}
\def\bR {{\Bbb R}} \def\bN {{\Bbb N}} \def\bZ {{\Bbb Z}}
\def\R {{\Bbb R}} \def\N {{\Bbb N}} \def\Z {{\Bbb Z}}
\def\B {{\Bbb B}} \def\C {{\Bbb C}} \def\D {{\Bbb D}}
\def\sA {{\cal A}} \def\sB {{\cal B}} \def\sC {{\cal C}}
\def\sD {{\cal D}} \def\sE {{\cal E}} \def\sF {{\cal F}}
\def\sG {{\cal G}} \def\sH {{\cal H}} \def\sI {{\cal I}}
\def\sJ {{\cal J}} \def\sK {{\cal K}} \def\sL {{\cal L}}
\def\sM {{\cal M}} \def\sN {{\cal N}} \def\sO {{\cal O}}
\def\sP {{\cal P}} \def\sQ {{\cal Q}} \def\sR {{\cal R}}
\def\sS {{\cal S}} \def\sT {{\cal T}} \def\sU {{\cal U}} 
\def\sV {{\cal V}} \def\sW {{\cal W}} \def\sX {{\cal X}} 
\def\sY {{\cal Y}} \def\sZ {{\cal Z}}

\def\q{\quad} \def\qq{\qquad}

\def \half {{\textstyle {1 \over 2}}}
\def\hhalf{{1/2}}
\def\fract#1#2{{\textstyle {#1\over #2}}}
\def\tfrac#1#2{{\textstyle {#1\over #2}}}
\def\qedi {\hfill\square\nl}
\def\qed {\hfill$\square$\par}
\def\llq {\lq\lq}
\def\rrq {\rq\rq{ }}
\def\BM {Brownian motion }
\def\PHI{{\mathop {{\rm PHI}}}}
\def\CS#1{\mathop {{\rm CS}(#1)}}
\def\betaloc{{\bar \beta}}

\def\tF{\widetilde F}
\def\hF{\widehat F}
\def\hX{\widehat X}


\def\dst{\displaystyle}
\def\tilzero{{\buildrel 0 \over \sim}}
\def\tilm{{ \; \buildrel m \over \sim \;}}
\def\tiln{{ \; \buildrel n \over \sim \;}}
\def\til-1{{\,\buildrel -1 \over \sim\,}}


\def\refer#1{ \medskip  \parindent=34pt \hang \noindent \rlap{[#1]\hfil} 
\hskip 30pt } 

\def\la{{\lambda}}
\def\lam{{\lambda}}
\def\th{{\theta}}
\def\al{{\alpha}}
\def\Gam{\Gamma}

\def\grad{{\nabla}}
\def\proof{{\medskip\noindent {\it Proof. }}}
\def\longproof#1{{\medskip\noindent {\bf Proof #1.}}}
\def\qed{{\hfill $\square$ \bigskip}}
\def\subsec#1{{\bigbreak\noindent \bf{#1}.}}
\def\blank#1{{\bigskip {\bf [#1]}\bigskip}}
\def\remark{{\noindent \bf Remark. }}
\def\bold{\bf}
\def\section#1#2{{\bigbreak\bigskip \centerline{\bf #1. #2}\bigskip}}
\def\notes{{\bigbreak\bigskip \centerline{\bf Notes}\bigskip}}
\def\cite#1{{[#1]}}
\def\figure#1{{\vglue2.1in\centerline{Figure #1}\bigskip}}
\def\ull{\hbox{\phantom{.}{\vrule width60pt }}\thinspace ,\ }

\def\eps{\varepsilon}
\def\vp{\varphi}
\def\vc{\overrightarrow}

\def\angel#1{{\langle#1\rangle}}
\def\pd {\partial}
\def\rowd#1#2{#1_1,\ldots,#1_{#2}}
\def\rowu#1#2{#1^1,\ldots,#1^{#2}}
\def\norm#1{\Vert #1 \Vert}
\def\emp {\emptyset}
\def\q {\quad} \def\qq {\qquad}
\def\frac#1#2{{#1\over #2}}
\def\ontop#1#2{{#1\atop #2}}
\def\del{{\partial}}
\def\wt{\widetilde}
\def\ol{\overline}
\def\oB{\ol B}
\def\wh{\widehat}
\def\lt{{\prec}}
\def\gt{{\succ}}
\def\absc{{\ll}}
\def\ni{\noindent}
\def\noi{\ni}
\def\ms{\medskip}
\def\bs{\bigskip}
\def\cl#1{\centerline{#1}}

\def\ftN{\rl\kern-0.13em\rN}

\def\Osc{\mathop {\rm Osc\, }}
\def\dist{{\mathop {{\rm dist\, }}}}
\def\diam{{\mathop {{\rm diam\, }}}}
\def\supp{{\mathop {{\rm supp\, }}}}
\def\div{{\mathop {{\rm div\, }}}}
\def\sgn{{\mathop {{\rm sgn\, }}}}
\def\Var{{\mathop {{\rm Var\, }}}}
\def\Cov{{\mathop {{\rm Cov\, }}}}
\def\inter{{\mathop {{\rm int\, }}}}
\def\clo{{\mathop {{\rm cl\,}}}}
\def\ae{{\rm a.e.\ }}
\def\as{{\rm a.s.\ }}
\def\io{{\rm i.o.\ }}
\def\ions{{\rm \  i.o.}}
\def\ae{{\rm a.e.\ }}
\def\BM{Brownian motion }
\def\sf{$\sigma$--field }
\def\e{{\cal E}}
\def\elt{{e^{-\lambda t}}}
\def\dnx{{D_n(x)}}
\def\snx{{\sigma_n(x)}}
\def\dnzx{{D_{n_0}(x)}}
\def\snzx{{\sigma_{n_0}(x)}}
\def\lex{{\lim_{\eps\to 0} \eps^{-d} \bE^x }}
\def\lf{l_{\cal F}} \def\mf{m_{\cal F}} \def\tf{t_{\cal F}} 
\def\rf{\rho_{\cal F}}
\def\bbe{\theta}  \def\dw{\beta} 
\def\ds{{d_s}} \def\df{{d_f}}
\def\ig{\sL}
\def\E{{\Bbb E}}
\def\P{{\Bbb P}}
\def \thalf {{\textstyle {1 \over 2}}}
\def\ra{\rightarrow}
\def\sDL{\sD(\sL)}
\def\dm {d\mu} \def\dmp{} 

\def\tlint{{- \kern-0.85em \int \kern-0.2em}}  % for textstyle
\def\dlint{{- \kern-1.05em \int \kern-0.4em}}  % for displays

%%%%Def from Martin's survey
\def\Lam {\Lambda}
\def\dg{d_G}
\def\wvp{\wh\vp}
\def\gam{\gamma}
\def\om{\omega}

\def\loc{{\rm loc}}
\def\Reff{R_{\rm eff}}
\def\PHI{\mathop{\hbox{PHI}}}
\def\EHI{\mathop{\hbox{EHI}}}
\def\VD{\mathop{\hbox{VD}}}
\def\PI{\mathop{\hbox{PI}}}
\def\CS{\mathop{\hbox{CS}}}
\def\CC{\mathop{\hbox{CC}}}
\def\HK{\mathop{\hbox{HK}}}
\def\RES{\mathop{\hbox{RES}}}
\def\div{{\mathop {{\rm div}}}}

%%%%New Def 
\def\es{\hbox{ess sup}}
\def\ei{\hbox{ess inf}}
\def\EE{\mathop{\hbox{E}}}

%%% Start of MSS

\font\titlefont=cmbx10 scaled\magstep2
                
\centerline {\titlefont Correction to \lq\lq Stability of parabolic
Harnack } 
\centerline {\titlefont inequalities on metric measure spaces''}
\medskip

\vskip .3truein

\centerline {Martin T. Barlow, 
\quad  Richard F. Bass \quad and \quad  Takashi Kumagai}

\vskip 0.3 truein

Dr. N. Kajino pointed us out that the proof of Lemma 3.3 in the paper [BBK] is inadequate,
since there is no easy way to control the Green function $g^D_\lam(x,y)$ near
the boundary of $D$. 
Since there are also some other minor errors in Section 3, we have made a revision from page 499,
 line 6 to the end of Section 3. We thank Dr. Kajino for pointing out the error and for his comments 
 on the revision. 

$$
---------------------------------------
$$

Let $Y$ be the process associated with the Dirichlet form $(\sE, \sF)$.
Let $G_\lam$ be the $\lam$-resolvent associated with the process $Y$; that is,
$$ G_\lam f(x) = \bE^x \int_0^{\infty} e^{-\lam t} f(Y_t) dt, $$
for bounded measurable $f$.  
Let $p_t(\cdot,\cdot)$ be the heat kernel of $Y$. 
Then the Green kernel of $G_\lam$ is given by
$$ g_\lam(x,y) =\int_0^\infty e^{-\lam t} p_t(x,y) dt.$$
We will use the Green kernel to build a cut-off function $\vp$. 

\proclaim Lemma 3.2. Let $x_0\in X$. Then there exist $\delta\in (0,1)$ 
and $C_1=C_1(\delta)>0$ such that if $\lam= c_0  \Psi (\delta R)^{-1}$, then   

$$ \eqalignno{ 
   &g_\lam(x,y) \le C_1 \frac{\Psi(R)}{V(x_0,R)}, \qq x \in  B(x_0,R)^c, \, y\in B(x_0,\delta R), &(3.1) \cr
  &g_\lam(x,y)  \ge 2C_1 \frac{\Psi(R)}{V(x_0,R)},  \qq x,y \in B(x_0,\delta R). &(3.2) 
 } $$

\proof This follows easily from $\HK(\Psi)$ by integration. \qed


\proclaim Lemma 3.3. 
There exists $\theta>0$ such that the following holds. 
Let $x_0 \in X$, $R>0$, $x_1 \in B(x_0,R)$, and $\lam \ge c \Psi(R)^{-1}$. Then
$$ |g_\lam(x_1,y)-g_\lam(x_1,y')| 
 \le c_1\Big(\frac{d(y,y')}{R}\Big)^{\th} \frac{ \Psi(R)} { V(x_0, R)}
 \q \hbox{ for } y,y'  \in B(x_0,2R)^c.  \eqno(3.3) $$

\proof If $d(y,y') \ge R/4$ then (3.3) follows immediately from (3.1). Otherwise 
we use the H\"older continuity of $p_t(x_1,\cdot)$, which follows from $\PHI(\Psi)$
by a standard argument; see [BGK], Corollary 4.2.  
(Note that to handle small values of $t$ 
we need to extend the function $p_\cdot(x_1,\cdot)$ from
$(0,\infty) \times B(x_0,R)^c$ to $\bR  \times B(x_0,R)^c$, by setting
$p_s(x_1,y)=0$ for $s<0$.) 
Once we have the H\"older continuity of $p_t(x_1,\cdot)$, 
integrating gives (3.3).  \qed

The following lemma is given in 
[BH] Chapter I, Proposition I.4.1.1 when $u, f\in \sF$ are non-negative and bounded, and
$f \ge 0$.
By a standard approximation argument, it can be proved for  the unbounded case as well. 

\proclaim Lemma 3.A. For $u\in \sF$, let $\Phi (u)=(u\vee 0)\wedge 1$. Then $\Phi (u)\in \sF$
and the following holds.
$$
\int_Xfd\Gamma(\Phi (u),\Phi (u))\le 
\int_Xfd\Gamma(u,u)\qquad~~\forall f\in \sF
~\hbox{ with }~ f\ge 0.
$$


Let $\delta$ be as in Lemma 3.2, 
fix $x_0\in X$ and let $B'=B(x_0,\delta R), B''=B(x_0,\delta R/8)$, $B=B(x_0,R)$, 
$2B=B(x_0,2R)$. By Remark 2.6(2-3) it is enough to prove  $\CS(\Psi)$ with
a scale factor of $\delta^{-1}$ rather than 2.

Let  
$\lambda =c_0\Psi(\delta R)^{-1}$ and define
$$
h:=C_1\Psi (R)\frac {V(x_0, \delta R/8)}{V(x_0, R)}.
$$
Integrating Lemma 3.2,  
we have the following:
$$ \eqalignno{ 
 &G_\lam1_{B''}(x) \le h, \qq x \in B(x_0, R)^c,  &(3.a) \cr
 &G_\lam1_{B''}(x) \ge 2h, \qq x \in B(x_0, \delta R), &(3.b)
 }$$
$$  |G_\lam1_{B''}(x)- G_\lam1_{B''}(y)| 
 \le c_1\Big(\frac{d(x,y)}{R}\Big)^{\th} h,~~x,y\in B(x_0,R)\setminus B(x_0,\delta R/2). 
 \eqno(3.c)$$

Now define 
$$\vp (x)=\Big(2\wedge h^{-1}G_{\lambda}1_{B''}(x)-1\Big)^+
=\Big(1\wedge (h^{-1}G_{\lambda}1_{B''}(x)-1)\Big)^+=\Phi(h^{-1}G_{\lambda}1_{B''}(x)-1).$$
We need to make sure that $\vp\in \sF$.
For the purpose, 
let $\hat 1_{B(x_1,s)}\in \sF\cap C_0$ be a function which is $1$ 
inside $B(x_1,s)$, between $0$ and $1$ in 
$B(x_1,2s)\setminus B(x_1,s)$ and $0$ outside $B(x_1,2s)$.  Then 
$h^{-1}G_{\lambda}1_{B''}(x)-1=
h^{-1}G_{\lambda}1_{B''}(x)-\hat 1_{2B}(x)$ for $x\in 2B$, so 
$$
\vp(x)=\Phi(h^{-1}G_{\lambda}1_{B''}(x)-1)=
\Phi(h^{-1}G_{\lambda}1_{B''}(x)-\hat 1_{2B}(x))\wedge \hat 1_{B}\in \sF.$$ 
Using (3.a)--(3.c), it is easy to check that 
$\vp$ is a cut-off function for $B'\subset B$ that satisfies 
Definition 2.5 (a)--(c). 
To complete the proof of $\CS(\Psi)$, we need to establish (2.5).

\proclaim Proposition 3.4. Let $x_1\in X$ and $f\in \sF$. 
Let $\delta$ be defined by Lemma 3.2 and let
$I=B(x_1,\delta s)$ with $0<s\le R$ and $I^*=B(x_1,s)$.  
There exist $c_1,c_2>0$ such that
for all $f\in \sF$,  
$$ \int_{I} f^2 d\Gam(\vp,\vp) \le c_1 (s/R)^{2\th} 
 \Big(  \int_{I^*} d\Gam(f,f) 
 + c_2 \Psi(s)^{-1} \int_{I^*} f^2d\mu \Big). \eqno(3.4) $$

\proof {\bf Step 1.}  We first prove that there exists a cutoff function
$\psi$ for $B' \subset B$, which we do not require  to be continuous,
 such that
$$  \int_{B} f^2 d\Gam(\psi,\psi) \le c_1  \Big(  \int_X d\Gam(f,f) 
 +  \Psi(R)^{-1} \int_X f^2d\mu \Big).   \eqno(3.d) $$ 
Let $D=B(x_0, R-\varepsilon)$ for some $\varepsilon>0$ and define 
$$ \sF_D = \{ f\in \sF: \wt f=0 \hbox { q.e. on } X-D \}. $$
Set
$$\sE_\lam(f,g)=\sE(f,g)+\lam \int fg\, d\mu.$$
Let $v= G_\lam^D 1_{B'}\in \sF$. Note that 
$$ v(x) \le \int_{B'}g^D(x,y)d\mu (y)\le \E^x[\tau_D]\le c \Psi(R), \qq x \in D,
\eqno(3.5)$$ by Theorem 2.15.
By [FOT] Theorem 4.4.1, $v\in  \sF_D$ and is quasi-continuous.
Further, since $Y$ is continuous, $v=0$ on $\ol D^c$.
Let $f\in \sF$. Then
$$ \int_B f^2 d\Gam(v,v) \le \int_X f^2 d\Gam(v,v) = 
 \int_X  d\Gam(f^2 v,v)   -\int_X 2fv  d\Gam(f,v). $$
Since $v \in \sF_D$ we have $f^2 v \in \sF_D$, so by
[FOT] Theorem 4.4.1,
$$  \int_X  d\Gam(f^2 v,v) = \sE(f^2 v,G^D_\lam 1_{B'}) 
 \le  \sE_\lam(f^2 v,G^D_\lam 1_{B'}) = \int_X f^2 v 1_{B'} d\mu
 \le c \Psi(R) \int_{B'} f^2 d\mu, $$
where we used (3.5) in the last inequality. 
Using Cauchy-Schwarz and (3.5), we obtain
$$ \eqalign{
 \Bigl|\int_X 2fv  d\Gam(f,v)\Bigr| &\le 
 c \Big(\int_X v^2 d\Gam(f,f) \Big)^{1/2} \Big(\int_X f^2 d\Gam(v,v) \Big)^{1/2} \cr
 &\le c \Psi(R) \Big(\int_B d\Gam(f,f) \Big)^{1/2} 
\Big(\int_X f^2 d\Gam(v,v) \Big)^{1/2}.\cr}$$


So, writing $H= \int_X f^2 d\Gam(v,v)$,  $J=\int_B d\Gam(f,f)$,
$K= \int_B f^2 d\mu$, we have
$$ H \le c \Psi(R) K + c \Psi(R) J^{1/2} H^{1/2}, $$
from which it follows that $H \le c \Psi(R) K + c\Psi(R)^2 J$.
{}
Let $\psi(x)=(v(x)/h)\wedge 1=\Phi(v(x)/h)$. 
Computing similarly to Lemma 3.2 using [BGK] Theorem 3.1, 
$\psi(x)=1$ for $x\in B(x_0,\delta R)$ so that $\psi$ is a cut-off function for $I\subset I^*$. Further, using 
Lemma 3.A, 
%Lemma 3.3, 
we have $\int_X f^2 d\Gam(\psi,\psi)\le h^{-2}H$. Thus (3.d) holds.

\nl {\bf Step 2.} 
In Step 2, we will consider the situation that either 
$$ I^* \subset B(x_0, \delta R) \eqno (3.6) $$
or else
$$  I^* \cap B(x_0, \delta R/2) =\emptyset . \eqno (3.7) $$
Since $\vp\equiv 1$ on $  B(x_0, \delta R)  $, (3.4) is clear if (3.6) holds. 
Thus, we consider when (3.7) holds. Let 
$\psi_s (x)$ be a cut-off function for $I\subset I^*$ given by Step 1. 
Let 
$\vp_0(x)= h^{-1}G_{\lambda}1_{B''}(x)\in \sF$,
$a_0 = \inf_{I^*} \vp_0$ and 
$\vp_1(x)=\vp_0(x)- a_0 \hat 1_{I^*}(x)\in \sF$.
Note that $\vp=\Phi (\vp_1 +a_0-1)$ on $I^*$. By 
(3.c) we have 
%(3.a) we have 
$$ \vp_1(x) \le c (s/R)^\th = L , \qq x\in I^*. $$
Let
$$\eqalign
{ A &=\int_{I} f^2 d\Gam(\vp,\vp), \cr
  D &= \int_{I^*} d\Gam(f,f)+ \Psi(s)^{-1} \int_{I^*}  f^2 d\mu,\cr
  F &=\int_{I^*} f^2 \psi_s^2  d\Gam(\vp_1,\vp_1). \cr}$$
By Lemma 3.A, we have
%By Lemma 3.3, we have
$$ \eqalignno{
 A& \le \int_{I} f^2 d\Gam(\vp_1,\vp_1)  \le  F= \int_{I^*} f^2 \psi_s^2 d\Gam(\vp_1,\vp_0)  \cr
  &=  \int_{I^*} d\Gam(f^2 \psi_s^2 \vp_1, \vp_0) 
  -  \int_{I^*} \vp_1 d\Gam(f^2 \psi_s^2 , \vp_0).   &(3.8) 
  }$$
For the first term in (3.8)
$$  \eqalign{ 
 \int_{I^*} d\Gam(f^2 \psi_s^2 \vp_1, \vp_0)
  &=   \int_{X} d\Gam(f^2 \psi_s^2 \vp_1, \vp_0) \cr
 &= \sE_\lam(f^2 \psi_s^2 \vp_1,  h^{-1}G_{\lambda}1_{B''}) 
- \lam\int_X f^2 \psi_s^2\vp_1 \vp_0 d\mu\cr
 &\le  \sE_\lam(f^2 \psi_s^2 \vp_1, h^{-1}G_{\lambda}1_{B''}) 
=  h^{-1}
\int_{B''} f^2 \psi_s^2 \vp_1d\mu =0. \cr }$$
Here we used the fact that  $\vp_1\ge 0$ on $I^*$ and 
that the support of $\psi_s$ is in $I^*$, hence outside $B''$ (due to (3.7)).

The final term in (3.8) is handled, using the Leibniz and chain rules and 
Cauchy-Schwarz, as
$$ \eqalign{
  &\Bigl| \int_{I^*} \vp_1 d\Gam(f^2 \psi_s^2, \vp_0) \Bigr|  
\le 2\Bigl| \int_{I^*} \vp_1f\psi_s^2 d\Gam(f , \vp_0) \Bigr|  +
2\Bigl| \int_{I^*} \vp_1f^2\psi_s d\Gam( \psi_s, \vp_0) \Bigr|  
\cr
 &\le c \Big\{ \Big(\int_{I^*} \psi_s^2  d\Gam(f,f) \Big)^{1/2}
 + \Big(\int_{I^*} f^2  d\Gam(\psi_s,\psi_s){\Big)}^{1/2} \Big\} 
   \Big( \int_{I^*} \vp_1^2 f^2 \psi_s^2 d\Gam(\vp_0,\vp_0)\Big)^{1/2} \cr
 &\le  c' D^{1/2} L  F^{1/2}, }$$ 
where we used Step 1 in the final line. 
Thus we obtain
$A\le F \le c DL^2$ so that (3.4) holds. 

\nl {\bf Step 3.} We finally consider the general case. 
When either (3.6) or (3.7) holds, the result is already proved in Step 2.
So assume that neither of them hold.
Then $I^*$ must intersect both $B(x_0,\delta R/2)$ 
and $B(x_0,\delta R)^c$, so $s\ge \delta R/4$.
We use Lemma 2.3 to cover 
$I$ with balls $B_i=B(x_i,c_1R)$, where $c_1\in (0, \delta/4)$
has been chosen small enough so that each 
$B_i^*:=B(x_i, c_1R/\delta)$  
satisfies at least one of (3.6) or (3.7). 
We can then apply (3.4) with $I$ replaced by each ball $B_i$:
writing $s'=c_1R$ we have
$$\int _{B_i} f^2 d\Gam(\vp,\vp) 
 \leq c_2(s'/R)^{2\th}  \Big(\int_{B^*_i} d\Gam(f,f)
+\Psi(s')^{-1} \int_{B^*_i} f^2d\mu\Big).$$
We then sum over $i$. Since no point
of $I^*$ is in more than $L_0$ (not depending on $x_0$ or $R$) 
of the $B^*_i$, and $c_1 s \le s'\le s$, we obtain (3.4) for $I$. \qed

\def \nr { \nl }
\bigbreak \centerline {\bf References}
\bigskip

\nr
[BBK] M.T. Barlow, R.F. Bass and T. Kumagai.  Stability of parabolic
Harnack inequalities on metric measure spaces. 
{\sl J. Math. Soc. Japan} (2) {\bf 58} (2006), 485--519.
\nr 
[BGK] M.T. Barlow, A. Grigor'yan and T. Kumagai.
On the equivalence of parabolic Harnack inequalities and heat kernel estimates.
{\it J. Math. Soc. Japan, \bf 64} (2012), 1091--1146. 
\nr 
[BH] N. Bouleau, F. Hirsch. 
{\sl Dirichlet forms and analysis on Wiener space.} de Gruyter, Berlin-New York, 1991.

\bye










